Learning-Based Image Compression for Machines

While learning based compression techniques for images have outperformed traditional methods, they have not been widely adopted in machine learning pipelines. This is largely due to lack of standardization and lack of retention of salient features needed for such tasks. Decompression of images have taken a back seat in recent years while the focus has shifted to an image's utility in performing machine learning based analysis on top of them. Thus the demand for compression pipelines that incorporate such features from images has become ever present. The methods outlined in the report build on the recent work done on learning based image compression techniques to incorporate downstream tasks in them. We propose various methods of finetuning and enhancing different parts of pretrained compression encoding pipeline and present the results of our investigation regarding the performance of vision tasks using compression based pipelines.

==> related_work.tex <==
Since the past several years various efforts have been made to achieve an efficient pipeline for compression based machine learning tasks and are often based on Neural Network architectures. 

\citet{https://doi.org/10.48550/arxiv.1802.01436} proposed an auto-encoder based network using a hyper-prior and GDN/IGDN modules for a better image compression. MS-SSIM was incorporated as the function that dictates the loss in the ANN modules. It achieved better performance scores for several image quality parameters like PSNR, than most contemporary ANN based modules and standards.

\citet{https://doi.org/10.48550/arxiv.2104.10065} introduced an effort towards JPEG-AI targeting texture recognition and proposed the use of cResNet-39 \cite{https://doi.org/10.48550/arxiv.1803.06131} to perform this task. They utilized HyperMS-SIM\cite{tfc_github} based compression technique and applied the cResNet-39 layers which are truncated ResNet-50 layers and fine-tuned them resulting in a comparable performance with respect to the anchors, showing how compressed domain from standard ANN based compression modules hold significant information for downstream ML tasks. 

\citet{https://doi.org/10.48550/arxiv.2206.05650} proposes a pre-processing enhanced compression pipeline for downstream machine vision tasks. Using a pre-processing module before the encoding on the image composed of a Unet-style architecture \cite{https://doi.org/10.48550/arxiv.1505.04597} for enhancing features in an image for downstream ML task. It utilized standard JPEG encoders for this task. Although, this technique compromises the utility of the pipeline for human perception of images. 

\citet{codevilla2021learned} introduces an end-to-end pipeline for certain machine vision downstream tasks adopting the hyper-prior encoder from \cite{https://doi.org/10.48550/arxiv.1802.01436}. They utilize an sResNet architecture after the encoding task and perform object classification, segmentation and detection on the compressed domain. This loss function as well as the rate/distortion loss for image reconstruction is used to train the network end-to-end. They show comparable results to state-of-the-art in the compressed domain. The proposed method in this paper will focus on several downstream tasks leading to an ed-to-end trained compression network while also exploring the tradeoff between machine vision tasks and human perception using a learned compressed domain. Thus filling in the performance and utilization gaps in the techniques mentioned. 
